Automatic Operator-level Parallelism Planning for Distributed Deep Learning -- A Mixed-Integer Programming Approach

As the artificial intelligence community advances into the era of large models with billions of parameters, distributed training and inference have become essential. While various parallelism strategies-data, model, sequence, and pipeline-have been successfully implemented for popular neural networks on main-stream hardware, optimizing the distributed deployment schedule requires extensive expertise and manual effort. Further more, while existing frameworks with most simple chain-like structures, they struggle with complex non-linear architectures. Mixture-of-experts and multi-modal models feature intricate MIMO and branch-rich topologies that require fine-grained operator-level parallelization beyond the capabilities of existing frameworks. We propose formulating parallelism planning as a scheduling optimization problem using mixed-integer programming. We propose a bi-level solution framework balancing optimality with computational efficiency, automatically generating effective distributed plans that capture both the heterogeneous structure of modern neural networks and the underlying hardware constraints. In experiments comparing against expert-designed strategies like DeepSeek's DualPipe, our framework achieves comparable or superior performance, reducing computational bubbles by half under the same memory constraints. The framework's versatility extends beyond throughput optimization to incorporate hardware utilization maximization, memory capacity constraints, and other considerations or potential strategies. Such capabilities position our solution as both a valuable research tool for exploring optimal parallelization strategies and a practical industrial solution for large-scale AI deployment.

==> extension_dynamic_loading.tex <==
\subsection*{Extension: Dynamic weight loading}
With the surging interest of deploying LLMs for small business or even personal use, a practical compromise is to dynamically loading and off-loading memory-consuming operation weights in the LLM during the process of of model training or inference, in so doing deploys the LLM at the cost of extra time. Some operations may share the same weights, such as layers in the same PP stage over different micro-batches. With a slight abuse of notations, we denote $W(w), \forall w \in \mathcal{W}$ as the size of weight $w$, while $Use(i,w)$ indicates whether operation $i$ uses weight $w$. Loading and off-loading an weight incurs time cost, denoted as $D_a^+$ and $D_a^-$, respectively. The decision involves whether to load weight $w$ before or unload the weight after executing operation (i), denoted as $l(i,w)$ and $ul(i,w)$, respectively, and $l_0(w,j)$ denotes whether to load weight $w$ onto machine $i$ before the main process starts. To monitor the presence of weights on the machines, we use $act^-(i,w)$ and $act^+(i,w)$ to denote if weight type $w$ is active before and after operation $i$, respectively. We use an auxiliary variable $first(i,j)$ to indicate the first operation on machine $j$. With the above additional quantities defined, we cast the scheduling problem with dynamic weight loading (FDJSSP-DL) as

\begin{align}
    & \noindent \nonumber \text{Eqs. \ref{obj:z}-\ref{cst:mem_def}, and} \\
    \label{cst:mem_init_rule_1}
    \begin{split}
        & M(1-first(,j)) + act^-(i,w) - l_0(w,j) \geq 0, \\ & \forall i, w, j
    \end{split} \\
    \label{cst:mem_init_rule_2}
    \begin{split}
        & - M(1-first(i,j)) + act^-(i,w) - l_0(w,j) \leq 0, \\  & \forall i, w, j
    \end{split} \\
    \label{cst:setup_rule_mandatory}
    & l(i,w) \geq  Use(i,w) (1- act^-(i,w)), \forall i \\
    \label{cst:activate_simulation_0}
    & act^+(i,w) = act^-(i,w) + l(i,w) - ul(i,w), \forall i,w \\
    \label{cst:activate_simulation_1}
    \begin{split}
        & M(1 - u(i_1,i_2)) + act^+(i_1,w) - act^-(i_2,w) \geq 0, \\ & \forall i_1 \neq i_2, \forall w
    \end{split}
     \\
    \label{cst:activate_simulation_2}
    \begin{split}
        & - M(1 - u(i_1,i_2)) + act^+(i_1,w) - act^-(i_2,w) \leq 0, \\ & \forall i_1 \neq i_2, \forall w
    \end{split}
\end{align}
where Eqs. \ref{cst:mem_init_rule_1}-\ref{cst:mem_init_rule_2} initializes the activation status of each layer weights at the start of the main process; Eqs. \ref{cst:setup_rule_mandatory} enforces presence of the required layer weights before each operation; Eqs. \ref{cst:activate_simulation_0}-\ref{cst:activate_simulation_2} simulate and monitor the activtaion status of layer weights according to the loading and off-loading decisions.


\subsection{Dynamic Parameter Loading}

o evaluate the effectiveness of our mathematical programming approach for automatic parallelization with dynamic parameter loading, we conducted experiments on a small-scale neural network training process. Figure \ref{example_dynamic_loading} presents the execution plan generated by our optimizer for a model with [number] parameters distributed across [number] computing nodes. We implemented our approach on a distributed cluster consisting of [number] nodes, each equipped with [specifications] and subject to a strict memory constraint of [X] GB per node. The target neural network architecture contained [details about model architecture] with a total parameter count of [number] million parameters. We used [dataset name] for the training process and measured the overall execution time, memory utilization, and computational efficiency.

As shown in Figure \ref{example_dynamic_loading}, our optimizer generated a non-trivial parallelization strategy that strategically schedules parameter loading and unloading operations to maximize computational efficiency while respecting memory constraints. The horizontal axis represents time progression during the training process, while the vertical axis shows the allocation of different model components across computing nodes.

Several key observations emerge from the visualization. 
Temporal Parameter Sharing: The optimizer dynamically redistributes parameters across nodes during different phases of training, effectively multiplexing the limited memory resources. This is evidenced by the frequent vertical transitions in the diagram, representing parameter movement operations.
Computation-Communication Overlap: The plan strategically schedules parameter loading operations (dotted lines becoming solid) to overlap with computation on other nodes, minimizing idle time during parameter transfers.
Memory Constraint Satisfaction: Throughout the execution, memory utilization on each node remains below the strict [X] GB threshold, as indicated by the controlled parameter loading patterns and the absence of excessive simultaneous activations on any single node.
Load Balancing: The optimizer achieves near-optimal load balancing across nodes, with computation time (solid colored segments) distributed evenly to avoid bottlenecks from overloaded nodes.
These results confirm that mathematical programming provides an effective framework for automating the complex decision-making process involved in parallelizing neural network training under strict memory constraints. The ability to dynamically load and unload parameters enables efficient training of larger models than would otherwise be possible on the same hardware configuration.

\begin{figure}[H]
\centering
\includegraphics[width=0.99\linewidth]{graph//dualpipe.png}\
\caption{Optimal parallel execution strategy for neural network training with dynamic parameter loading on a memory-constrained distributed cluster. The visualization illustrates the time-dependent allocation of model components across computing nodes, showing parameter loading/unloading events (vertical transitions) and computation phases (horizontal segments). Different colors represent distinct model components, with solid lines indicating active computation and dotted lines representing loaded but idle parameters. This automatically generated parallelization plan minimizes total training time while respecting strict per-node memory constraints of [X] GB.}
\label{example_dynamic_loading}
\end{figure}
